The Matrix of Linear Mappings

On the set of mappings of the given set, we define the product of mappings. If A is associative algebra, then we consider the set of matrices, whose elements are linear mappings of algebra A. In algebra of matrices of linear mappings we define the operation of product. The operation is based on the product of mappings. If the matrix a of linear mappings has an inverse matrix, then the quasideterminant of the matrix a and the inverse matrix are matrices of linear mappings. In the paper, I consider conditions when a matrix of linear mappings has inverse matrix, as well methods of solving a system of linear equations in an associative algebra.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{Weinberg}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Greiner Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem
{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов, Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин,
Элементы теории функций и функционального анализа,
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том 1, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

%\BiblioItem{Kleyn} http://www.geocities.com/aleks\_kleyn/Derivative/Derivative.htm

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Muller}
{
Holger Muller et al.,
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators,
\href{http://prola.aps.org/searchabstract/PRL/v91/i2/e020401}{Phys. Rev. Lett. 91, 020401} (2003),
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2000)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem
{q-alg-9705026}
{
I.Gelfand, V.Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
I. Gelfand and V. Retakh, Determinants of Matrices over Noncommutative Rings, Funct.
Anal. Appl. 25 (1991), no. 2, 91-102
}%

\BiblioItem{Gelfand Retakh 1992}
{
I. Gelfand and V. Retakh, A Theory of Noncommutative Determinants and Characteristic
Functions of Graphs, Funct. Anal. Appl. 26 (1992), no. 4, 1-20
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2009)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2009)
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология, Использование вещественных чисел в общей топологии,
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М. Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{Convention.Eq}

\section{Соглашения}

\begin{enumerate}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315}
\ifx\Semafor\ValueOn
\item Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции.
%Однако мы можем рассматривать свободную
%алгебру как векторное пространство над полем.
%Так как нежелательно одно и тоже соответствие называть то функцией, то
%отображением, я буду пользоваться термином линейная функция алгебры.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,Report.10,1001.4852}
\ifx\Semafor\ValueOn
\item
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061}
\ifx\Semafor\ValueOn
\item
В выражении вида
\[
\pC s0a\ x\ \pC s1a
\]
предполагается сумма по индексу $s$.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\item
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
При этом подразумевается, что отображение мультипликативно над
максимально возможным полем. В частности, линейное отображение
тела $D$ мультипликативно над центром $Z(D)$. Это не противоречит
определению линейного отображения поля, так как для поля $F$ справедливо
$Z(F)=F$.
Если поле $F$ отлично
от максимально возможного, то я это явно указываю в тексте.
\fi

\ePrints{0912.4061,Report.10}
\ifx\Semafor\ValueOn
\item
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307}
\ifx\Semafor\ValueOn
\item
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061,1001.4852}
\ifx\Semafor\ValueOn
\item Мы будем рассматривать алгебру $A$, которая является конечно
мерным векторным пространством над центром.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
Однако в алгебре не принято использовать векторные обозначения.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}

\item При рассмотрении конечномерной алгебры мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\fi

\ePrints{0906.0135,0912.3315}
\ifx\Semafor\ValueOn
\item
Так как число $\mathfrak{F}$\Hyph алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\mathfrak{F}_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\mathfrak{F}}$\Hyph алгебр.
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом $\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\mathfrak{F}}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\Vector A_{[1]},\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.

\item Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\item
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\fi

\item
Без сомнения, у читателя моих статей могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.

\end{enumerate}



==> Function.Matrix.Russian.tex <==
%auto-ignore
\input{Function.Matrix.Eq}

\section{Произведение отображений}

На множестве отображений
\ShowEq{set of mappings A}
определено произведение согласно правилу
\ShowEq{set of mappings A, product}
Равенство
\ShowEq{f circ g = g circ f}
справедливо тогда и только тогда, когда диаграма
\ShowEq{f circ g = g circ f, diagram}
коммутативна.

Для $a\in A$, существует отображение
\ShowEq{mapping f a=a}
Если мы будем обозначать отображение $f_a$ буквой $a$,
то опираясь на равенство
\eqref{eq: set of mappings A, product},
положим
\ShowEq{set of mappings A, product over scalar}

\section{Бикольцо функциональных матриц}

Если $A$ - $\mathfrak{H}$\Hyph алгебра
(\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}),
в которой определена операция сложения,
то мы рассмотрим множество
\AddIndex{функциональных матриц}{functional matrix},
элементы которых
являются отображения
\ShowEq{set of mappings A}
Согласно определению
\xRef{0701.238}{definition: rc-product of matrices},
мы определим
\AddIndex{$\RCcirc$\Hyph произведение функциональных матриц}
{rc product of functional matrices}
\ShowEq{rc product of functional matrices}
Согласно определению
\xRef{0701.238}{definition: cr-product of matrices},
мы определим
\AddIndex{$\CRcirc$\Hyph произведение функциональных матриц}
{cr product of functional matrices}
\ShowEq{cr product of functional matrices}

\ifx\texFuture\Defined
\begin{definition}
Пусть $A$ - $\mathfrak{H}$\Hyph алгебра.
Тогда на множестве $A^n$ можно определить структуру
$\mathfrak{H}$\Hyph алгебры таким образом, что все операции
выполняются покомпонентно. А именно,
если $\omega$ - $p$\Hyph арная операция,
то для заданных кортежей
\ShowEq{Cartesian power of algebra, 1}
действие операции $\omega$ определено согласно правилу
\ShowEq{Cartesian power of algebra, 2}
$\mathfrak{H}$\Hyph алгебра $A^n$ называется
\AddIndex{декартовой степенью $n$ $\mathfrak{H}$\Hyph алгебры}
{Cartesian power of algebra} $A$.
\qed
\end{definition}

\begin{definition}
Пусть $A$ - $\mathfrak{H}$\Hyph алгебра,
в которой определена операция сложения.
Функциональная матрица $a$ называется
\AddIndex{матрицей эндоморфизмов $\mathfrak{H}$\Hyph алгебры}
{matrix of endomorphisms of H algebra}
$A$, если $a_i^j$ является эндоморфизмом $\mathfrak{H}$\Hyph алгебры $A$.
\qed
\end{definition}

\begin{theorem}
Пусть $A$ - $\mathfrak{H}$\Hyph алгебра,
в которой определена операция сложения.
$n\times n$ матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
является эндоморфизмом $\mathfrak{H}$\Hyph алгебры $A^n$.
\end{theorem}
\begin{proof}
Пусть $f$ - матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$.
Тогда для
\ShowEq{matrix of endomorphism, 1}
Если $\omega$ - $p$\Hyph арная операция, то
\ShowEq{matrix of endomorphism, 2}
\end{proof}

\begin{theorem}
$\RCcirc$\Hyph произведение матриц эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
является матрицей эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$.
\end{theorem}
\begin{proof}
Пусть $f$, $g$ - матрицы эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$.
Тогда для операции $\omega$ справедливо равенство
\ShowEq{matrix of endomorphism, 3}
\end{proof}

\begin{theorem}
Если произведение эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
ассоциативно,
то произведение матриц эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
ассоциативно.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из цепочки равенств
\ShowEq{product of matrices of endomorphisms is associative}
\end{proof}

\section{Квазидетерминант матрицы эндоморфизмов}

\begin{theorem}
\label{theorem: rc inverse minor, matrix of endomorphisms}
Предположим, что $n\times n$ матрица $a$
эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
имеет $\RCcirc$\Hyph обратную матрицу\footnote{Это утверждение
и его доказательство основаны
на утверждении 1.2.1 из \citeBib{math.QA-0208146}
(\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=8}{page 8})
для матриц над свободным кольцом с делением.}
\ShowEq{rc inverce matrix of endomorphisms, definition}
Тогда $k\times k$ минор $\RCcirc$\Hyph обратной матрицы
удовлетворяет следующему равенству, при условии, что рассматриваемые
обратные матрицы существуют,\footnote{
Запись
\ShowEq{index of inverse element, 1}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать это выражение следующим образом
\ShowEq{index of inverse element, 2}
}
\ShowEq{rc inverse minor, matrix of endomorphisms}
\end{theorem}
\begin{proof}
Определение \eqref{eq: rc inverce matrix of endomorphisms, definition}
$\RCcirc$\Hyph обратной матрицы
приводит к системе линейных уравнений
\ShowEq{rc inverse minor, matrix of endomorphisms, 1}
Мы умножим \eqref{eq: rc inverse minor, matrix of endomorphisms, 1, 1} на
\ShowEq{rc inverse minor, matrix of endomorphisms, 3}
Теперь мы можем подставить
\eqref{eq: rc inverse minor, matrix of endomorphisms,3} в
\eqref{eq: rc inverse minor, matrix of endomorphisms, 1, 2}
\ShowEq{rc inverse minor, matrix of endomorphisms, 4}
\eqref{eq: rc inverse minor, matrix of endomorphisms}
следует из \eqref{eq: rc inverse minor, matrix of endomorphisms,4}.
\end{proof}

\begin{corollary}
\label{corollary: rc inverse matrix of endomorphisms}
Предположим, что $n\times n$ матрица $a$
эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$
имеет $\RCcirc$\Hyph обратную матрицу.
Тогда элементы $\RCcirc$\Hyph обратной матрицы удовлетворяют
равенству\footref{footnote: index of inverse element}
\ShowEq{rc inverse matrix of endomorphisms}
\qed
\end{corollary}

\begin{definition}
\label{definition: rc-quasideterminant, matrix of endomorphisms}
\AddIndex{$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант}
{a b RCcirc-quasideterminant}
$n\times n$ матрицы $a$
- это формальное выражение\footref{footnote: index of inverse element}
\ShowEq{a b RCcirc-quasideterminant definition}
Согласно замечанию
\xRef{0701.238}{remark: combine the notation of indexes}
мы можем рассматривать $(^b_a)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RCcirc-quasideterminant definition},
которую мы будем называть
\AddIndex{$\RCcirc$\Hyph квазидетерминантом}
{RCcirc-quasideterminant definition}.
\qed
\end{definition}

\begin{theorem}
Выражение для элементов $\RCcirc$\Hyph обратной матрицы имеет вид
\ShowEq{quasideterminant and inverse, RCcirc}
\end{theorem}
\begin{proof}
\eqref{eq: quasideterminant and inverse, RCcirc} следует
из \eqref{eq: a b RCcirc-quasideterminant definition}.
\end{proof}

\begin{theorem}
Выражение для
$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант
имеет любую из следующих форм
\ShowEq{RCcirc quasideterminant, expression}
\end{theorem}
\begin{proof}
Утверждение  следует
из \eqref{eq: rc inverse matrix of endomorphisms} и
\eqref{eq: a b RCcirc-quasideterminant definition}.
\end{proof}
\fi

\section{Алгебра линейных отображений}

Пусть $A$ - ассоциативная алгебра над полем $F$.
Пусть $\Basis e$ - базис алгебры $A$ над полем $F$.
Пусть $\Vector e_{\gi 0}$ - единица алгебры $A$.
Произведение в алгебре $A$ определено согласно правилу
\ShowEq{product in associative algebra}

Из равенства
\ShowEq{associative product in algebra}
следует равенство
\ShowEq{associative product in algebra, 1}

Для заданных $a$, $b\in A$ определено линейное отображение
$a\otimes b$ согласно правилу
\ShowEq{linear mapping of algebra, a b}
Сумма линейных отображений также является линейным отображением.
Множество линейных отображений является алгеброй $A\otimes A$.
Произведение в алгебре $A\otimes A$ определено согласно
правилу
\ShowEq{linear mapping of algebra, product}
Равенство \eqref{eq: linear mapping of algebra, product}
следует из равенства
\ShowEq{linear mapping of algebra, product 1}

В дальнейшем мы будем пользоваться стандартным представлением
\ShowEq{linear mapping of algebra, standard representation}

\begin{theorem}
Произведение линейных отображений, заданных в стандартном представлении,
имеет вид
\ShowEq{linear mapping of algebra, standard representation, product}
\end{theorem}
\begin{proof}
Утверждение теоремы следует из равенства
\ShowEq{linear mapping of algebra, standard representation, product 1}
\end{proof}

\begin{theorem}
\label{theorem: product of linear mappings is associative}
Произведение линейных отображений алгебры $A$
ассоциативно.
\end{theorem}
\begin{proof}
Рассмотрим линейные отображения
\ShowEq{linear mapping of algebra, product associative, 1}
Согласно равенству
\eqref{eq: linear mapping of algebra, standard representation, product}
\ShowEq{linear mapping of algebra, product associative, 2}
Согласно равенству
\eqref{eq: associative product in algebra, 1}
\ShowEq{linear mapping of algebra, product associative, 3}
Утверждение теоремы следует из равенств
\eqref{eq: linear mapping of algebra, product associative, 2 1},
\eqref{eq: linear mapping of algebra, product associative, 2 2},
\eqref{eq: linear mapping of algebra, product associative, 3 1},
\eqref{eq: linear mapping of algebra, product associative, 3 2}.
\end{proof}

\section{Матрица линейных отображений}

Пусть $A$ - ассоциативная алгебра над полем $F$.

\begin{definition}
Функциональная матрица $a$ называется
\AddIndex{матрицей линейных отображений}
{matrix of linear mappings},
если $a_i^j$ является линейным отображением алгебры $A$.
\qed
\end{definition}

\begin{theorem}
Произведение матриц линейных отображений алгебры $A$
ассоциативно.
\end{theorem}
\begin{proof}
Утверждение теоремы следует из теоремы
\ref{theorem: product of linear mappings is associative}
и цепочки равенств
\ShowEq{product of matrices of endomorphisms is associative}
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
$n\times n$ матрица линейных отображений алгебры $A$
является матрицей линейного отображения
векторного пространства над алгеброй $A$.
\end{theorem}
\begin{proof}
Пусть $f$ - матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры $A$.
Тогда для
\ShowEq{matrix of endomorphism, 1}
Если $\omega$ - $p$\Hyph арная операция, то
\ShowEq{matrix of endomorphism, 2}
\end{proof}
\fi

\begin{theorem}
$\RCcirc$\Hyph произведение матриц линейных отображений
является матрицей линейных отображений.
\end{theorem}
\begin{proof}
Следствие равенства
\eqref{eq: rc product of functional matrices}
и теоремы
\xRef{0701.238}{theorem: product of additive map, D D D}.
\end{proof}

Для записи линейного отображения мы будем пользоваться
стандартным представлением.
Стандартное представление матрицы линейных отображений имеет вид
\ShowEq{linear matrix, standard representation}
Согласно определению
\eqref{eq: set of mappings A, product over scalar},
\ShowEq{linear matrix, standard representation, RCcirc product}

\begin{theorem}
\label{theorem: linear matrices B rc C}
Для заданных матриц линейных отображений
\ShowEq{linear matrices B C}
$\RCcirc$\Hyph произведение имеет вид
\ShowEq{linear matrices B rc C}
\end{theorem}
\begin{proof}
Из равенства
\eqref{eq: cr product of functional matrices}
следует
\ShowEq{linear matrices B rc C, 1}
Равенство
\eqref{eq: linear matrices B rc C}
следует из равенства
\eqref{eq: linear matrices B rc C, 1}.
\end{proof}

\section{Квазидетерминант матрицы линейных отображений}

\begin{theorem}
\label{theorem: rc inverse minor, matrix of linear mappings}
Предположим, что $n\times n$ матрица $a$
линейных отображений алгебры $A$
имеет $\RCcirc$\Hyph обратную матрицу\footnote{Это утверждение
и его доказательство основаны
на утверждении 1.2.1 из \citeBib{math.QA-0208146}
(\href{http://arxiv.org/PS_cache/math/pdf/0208/0208146.pdf\#Page=8}{page 8})
для матриц над свободным кольцом с делением.}
\ShowEq{rc inverce matrix of endomorphisms, definition}
Тогда $k\times k$ минор $\RCcirc$\Hyph обратной матрицы
удовлетворяет следующему равенству, при условии, что рассматриваемые
обратные матрицы существуют,\footnote{
Запись
\ShowEq{index of inverse element, 1}
означает, что
при обращении Адамара столбцы и строки меняются местами.
\label{footnote: index of inverse element}
Мы можем
формально записать это выражение следующим образом
\ShowEq{index of inverse element, 2}
}
\ShowEq{rc inverse minor, matrix of endomorphisms}
\end{theorem}
\begin{proof}
Определение \eqref{eq: rc inverce matrix of endomorphisms, definition}
$\RCcirc$\Hyph обратной матрицы
приводит к системе линейных уравнений
\ShowEq{rc inverse minor, matrix of endomorphisms, 1}
Мы умножим \eqref{eq: rc inverse minor, matrix of endomorphisms, 1, 1} на
\ShowEq{rc inverse minor, matrix of endomorphisms, 3}
Теперь мы можем подставить
\eqref{eq: rc inverse minor, matrix of endomorphisms,3} в
\eqref{eq: rc inverse minor, matrix of endomorphisms, 1, 2}
\ShowEq{rc inverse minor, matrix of endomorphisms, 4}
\eqref{eq: rc inverse minor, matrix of endomorphisms}
следует из \eqref{eq: rc inverse minor, matrix of endomorphisms,4}.
\end{proof}

\begin{corollary}
\label{corollary: rc inverse matrix of linear mappings}
Предположим, что $n\times n$ матрица $a$
линейных отображений алгебры $A$
имеет $\RCcirc$\Hyph обратную матрицу.
Тогда элементы $\RCcirc$\Hyph обратной матрицы удовлетворяют
равенству\footref{footnote: index of inverse element}
\ShowEq{rc inverse matrix of endomorphisms}
\qed
\end{corollary}

\begin{definition}
\label{definition: rc-quasideterminant, matrix of endomorphisms}
\AddIndex{$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант}
{a b RCcirc-quasideterminant}
$n\times n$ матрицы $a$
- это формальное выражение\footref{footnote: index of inverse element}
\ShowEq{a b RCcirc-quasideterminant definition}
Согласно замечанию
\xRef{0701.238}{remark: combine the notation of indexes}
мы можем рассматривать $(^b_a)$\hyph \RC квазидетерминант
как элемент матрицы
\ShowEq{RCcirc-quasideterminant definition},
которую мы будем называть
\AddIndex{$\RCcirc$\Hyph квазидетерминантом}
{RCcirc-quasideterminant definition}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: quasideterminant and inverse, RCcirc}
Выражение для элементов $\RCcirc$\Hyph обратной матрицы имеет вид
\ShowEq{quasideterminant and inverse, RCcirc}
\end{theorem}
\begin{proof}
\eqref{eq: quasideterminant and inverse, RCcirc} следует
из \eqref{eq: a b RCcirc-quasideterminant definition}.
\end{proof}

\begin{theorem}
Выражение для
$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант
имеет любую из следующих форм
\ShowEq{RCcirc quasideterminant, expression}
\end{theorem}
\begin{proof}
Утверждение  следует
из \eqref{eq: rc inverse matrix of endomorphisms} и
\eqref{eq: a b RCcirc-quasideterminant definition}.
\end{proof}

\begin{theorem}
\label{theorem: quasideterminant of matrix of linear mappings}
Пусть $a$ - матрица линейных отображений.
Тогда матрицы
$\det\left(a,\RCcirc\right)$ и
$a^{-1\RCcirc}$ являются
матрицами линейных отображений.
\end{theorem}
\begin{proof}
Мы докажем теорему индукцией по порядку матрицы.

При $n=1$ из равенства
\eqref{eq: RCcirc quasideterminant, expression, 1}
следует
\ShowEq{quasideterminant of matrix of linear mappings, 1}
Следовательно, квазидетерминант является матрицей
линейных отображений.
Из теоремы
\xRef{0912.4061}{theorem: linear equation in associative algebra, root}
следует, что матрица $a^{-1\RCcirc}$ является
матрицей линейных отображений.

Пусть утверждение теоремы верно для $n-1$.
Пусть $a$ - $n\times n$ матрица.
Согласно предположению индукции, матрица
\ShowEq{minor of RCcirc quasideterminant}
в равенстве
\eqref{eq: RCcirc quasideterminant, expression, 1}
является матрицей линейных отображений.
Следовательно,
$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант
является линейным отображением.
Из теорем
\xRef{0912.4061}{theorem: linear equation in associative algebra, root},
\ref{theorem: quasideterminant and inverse, RCcirc}
следует, что матрица $a^{-1\RCcirc}$ является
матрицей линейных отображений.
\end{proof}

\section{Система линейных уравнений в ассоциативной алгебре}

\begin{theorem}
\label{theorem: standard identity matrix}
Единичная матрица $e$ имеет стандартное представление
\ShowEq{standard identity matrix}
\end{theorem}
\begin{proof}
Прежде всего, элементы единичной матрицы отличны от $0$ только
на диагонали. Следовательно, $i=j$.
Так как каждый элемент на диагонали равен единице поля, то
элемент матрицы имеет вид
$\Vector e_{\gi 0}\otimes\Vector e_{\gi 0}$.
Следовательно, $\gi k=\gi 0$, $\gi m=\gi 0$.
\end{proof}

\begin{theorem}
\label{theorem: inverce linear matrix}
Пусть $a$ - матрица линейных отображений алгебры $A$.
Пусть $b$ - матрица, $\RCcirc$\Hyph обратная матрице $a$.
Элементы матриц $a$ и $b$ связаны уравнением
\ShowEq{inverce linear matrix}
\end{theorem}
\begin{proof}
Равенство
\eqref{eq: inverce linear matrix}
является следствием равенств
\eqref{eq: linear matrices B rc C},
\eqref{eq: standard identity matrix}.
\end{proof}

\begin{definition}
Если $n\times n$ матрица $a$
линейных отображений алгебры $A$ имеет
$\RCcirc$\Hyph обратную матрицу,
мы будем называть матрицу $a$
\AddIndex{$\RCcirc$\Hyph невырожденной матрицей линейных отображений}
{RCcirc nonsingular matrix of linear mappings}.
В противном случае, мы будем называть такую матрицу
\AddIndex{$\RCcirc$\Hyph вырожденной матрицей линейных отображений}
{RCcirc singular matrix of linear mappings}.
\qed
\end{definition}

Система линейных уравнений в ассоциативной алгебре
имеет вид
\ShowEq{system of linear equations in associative algebra}
Мы можем записать систему линейных уравнений
\eqref{eq: system of linear equations in associative algebra}
в матричной форме
\ShowEq{system of linear equations in associative algebra, matrix}

\begin{definition}
Предположим, что $a$
- $\RCcirc$\Hyph невырожденная матрица. Мы будем называть
соответствующую систему
линейных уравнений
\eqref{eq: system of linear equations in associative algebra, matrix, 2}
\AddIndex{$\RCcirc$\Hyph невырожденной системой линейных уравнений}
{RCcirc nonsingular system of linear equations}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: nonsingular system of linear equations in algebra}
Решение невырожденной системы линейных уравнений
\eqref{eq: system of linear equations in associative algebra, matrix, 2}
определено однозначно
и может быть записано в любой из следующих форм
\ShowEq{nonsingular system of linear equations in algebra}
\end{theorem}
\begin{proof}
Умножая обе части равенства
\eqref{eq: system of linear equations in associative algebra, matrix, 2}
слева на $a^{-1\RCcirc}$, мы получим
\eqref{eq: nonsingular system of linear equations in algebra, solution, matrix}.
Пользуясь определением
\eqref{eq: a b RCcirc-quasideterminant definition},
мы получим \eqref{eq: nonsingular system of linear equations in algebra, solution, quasideterminant}.
%Решение системы единственно в силу теоремы
%\xEqRef{0612.111}{theorem: two products equal}.
\end{proof}

Мы можем также рассмотреть решение
системы линейных уравнений
\eqref{eq: system of linear equations in associative algebra, matrix, 1}
аналогично тому, как это сделано в теореме
\xRef{0912.4061}
{theorem: determinant of linear equation in associative algebra over field}
Если $a^k$ имеет разложение
\ShowEq{ak expansion basis e}
то система линейных уравнений
\eqref{eq: system of linear equations in associative algebra}
эквивалентна системе линейных уравнений
\ShowEq{system of linear equations in associative algebra, basis}
где
\ShowEq{system of linear equations in associative algebra, basis, 1}

\ifx\texFuture\Defined
Однако нас интересует решение системы линейных уравнений, оставаясь
в рамках алгебры $A$.

Рассмотрим систему двух линейных уравнений с двумя неизвестными.
Эту систему можно записать в виде
\ShowEq{system of linear equations in associative algebra, 2}
Мы можем записать систему линейных уравнений
\eqref{eq: system of linear equations in associative algebra, 2}
в матричной форме
\ShowEq{system of linear equations in associative algebra, matrix, 2}

показать, что если система имеет единственное решение, то по крайней
мере одна из функций $f^1_1$, $f^2_1$ обратима.
\fi


==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-drc форма
   {$1$-\drc форма}%
   {1-drc form, vector spaces}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%596%A%a b RCcirc квазидетерминант
   {$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {a b RCcirc-quasideterminant}%
\Index%3%A%a b-CR квазидетерминант
   {$(^a_b)$\hyph \CR квазидетерминант}%
   {a b cr-quasideterminant}%
\Index%4%A%a b-RC квазидетерминант
   {$(^a_b)$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%581%A%Arc  линейно зависимые векторы
   {$A\RCstar$\Hyph  линейно зависимые векторы}%
   {linearly dependent, A vector space}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%580%A%Arc линейно независимые векторы
   {$A\RCstar$\Hyph линейно независимые векторы}%
   {linearly independent, A vector space}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение функциональных матриц
   {$\CRcirc$\Hyph произведение функциональных матриц}%
   {cr product of functional matrices}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%13%C%crd производная Гато отображения \Vector f D-векторного пространства \Vector V в D-векторное пространство \Vector W
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%16%D%dcr базис векторного пространства c строк
   {\dcr базис векторного пространства \subs строк}%
   {dcr basis, c rows vector space}%
\Index%17%D%dcr вектор
   {\dcr вектор}%
   {dcr vector}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%19%D%dcr векторное пространство c строк
   {\dcr векторное пространство \subs строк}%
   {subs rows dcr vector space}%
\Index%20%D%Drc  линейно зависимые векторные поля
   {\Drc  линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%D%drc  линейно зависимые векторы
   {\drc  линейно зависимые векторы}%
   {linearly dependent, vector space}%
\Index%22%D%drc автоморфизм векторного пространства
   {\drc автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%111%D%drc аффинный базис
   {\drc аффинный базис}%
   {drc affine basis, division ring}%
\Index%24%D%drc базис в векторном пространстве
   {\drc базис в векторном пространстве}%
   {drc basis, vector space}%
\Index%25%D%drc базис в векторном пространстве r строк
   {\drc базис в векторном пространстве \sups строк}%
   {drc basis, r rows vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%27%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%29%D%drc векторное пространство r строк
   {\drc векторное пространство \sups строк}%
   {sups rows drc vector space}%
\Index%30%D%drc вектор-функция
   {\drc вектор\hyph функция}%
   {drc vector function}%
\Index%31%D%drc изоморфизм векторных пространств
   {\drc изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%32%D%drc линейная оболочка в векторном пространстве
   {\drc линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Index%33%D%Drc линейно независимые векторные поля
   {\Drc линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%34%D%drc линейно независимые векторы
   {\drc линейно независимые векторы}%
   {linearly independent, vector space}%
\Index%35%D%drc линейное отображение векторных пространств
   {\drc линейное отображение векторных пространств}%
   {drc linear map of vector spaces}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%37%D%drc линейным starT- представление группы
   {\drc линейным \sT представление группы}%
   {drc linear starT representation of group}%
\Index%38%D%drc производная Гато отображения \Vector f D- векторного пространства \Vector V в D- векторное пространство \Vector W
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%42%D%Dstar компонента координат вектора \Vector r
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\Index%51%E%essential parameters
   {essential parameters}%
   {essential parameters}%
\SetIndexSpace%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis\ векторного пространства
   {\Gbasis\ векторного пространства}%
   {G-basis}%
\Index%54%G%G-coords ы базиса
   {\Gcoords ы базиса}%
   {G-coordinates}%
\Index%55%G%G-space о
   {\Gspace о}%
   {GSpace}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главный минор
   {\RC главный минор}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%273%R%RC невырожденная система drc линейных уравнений
   {\RC невырожденная система \drc линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение функциональных матриц
   {$\RCcirc$\Hyph произведение функциональных матриц}%
   {rc product of functional matrices}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица линейных отображений
   {$\RCcirc$\Hyph вырожденная матрица линейных отображений}%
   {RCcirc singular matrix of linear mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица линейных отображений
   {$\RCcirc$\Hyph невырожденная матрица линейных отображений}%
   {RCcirc nonsingular matrix of linear mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система линейных уравнений
   {$\RCcirc$\Hyph невырожденная система линейных уравнений}%
   {RCcirc nonsingular system of linear equations}%
\Index%49%R%rcd базис, дуальный drc базису в векторном пространстве
   {\rcd базис, дуальный \drc базису в векторном пространстве}%
   {basis dual to basis, drc vector space}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%70%R%rcd представление группы
   {\rcd представление группы}%
   {rcd linear representation of group}%
\Index%71%R%Rstar- модуль
   {$R\star$\Hyph модуль}%
   {Rstar-module}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\SetIndexSpace%
\Index%73%S%SRCstar,TRCstar- линейное отображение векторных пространств
   {$(S\RCstar,T\RCstar)$\Hyph линейное отображение векторных пространств}%
   {src trc linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%586%S%star A- product of Astar linear map over scalar
   {$\star A$\Hyph произведением $A\star$\Hyph линейного отображения на скаляр}%
   {starA product of Astar linear map over scalar}%
\Index%77%S%star D- произведением drc линейного отображения A на скаляр
   {$\star D$\Hyph произведением \drc линейного отображения $A$ на скаляр}%
   {starD product of drc linear map over scalar}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%75%S%starD компонента координат вектора \Vector r
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%82%S%starT- представление \mathfrak{F}- алгебры A в H алгебре M
   {\sT представление $\mathfrak{F}$\Hyph алгебры $A$ в $\mathfrak{H}$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной \mathfrak{F}- алгебры
   {\sT представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {starT representation of fibered F-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%88%T%Tstar- линейная комбинация векторов
   {\Ts линейная комбинация векторов}%
   {linear composition of  vectors}%
\Index%90%T%Tstar- представление \mathfrak{F}- алгебры A в H алгебре M
   {\Ts представление $\mathfrak{F}$\Hyph алгебры $A$ в $\mathfrak{H}$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной \mathfrak{F}- алгебры
   {\Ts представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {Tstar representation of fibered F-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления F алгебры
   {автоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%96%А%аддитивное отображение D- векторных пространств
   {аддитивное отображение $D$\Hyph векторных пространств}%
   {additive map of D vector spaces}%
\Index%97%А%аддитивное отображение кольца
   {аддитивное отображение кольца}%
   {Additive map of Ring}%
\Index%98%А%аддитивное отображение тела, порождённое отображением G
   {аддитивное отображение тела, порождённое отображением $G$}%
   {additive map generated by map, division ring}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%569%А%активное представление лупы в многообразии базисов
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве drc базисов
   {активное преобразование на множестве \drc базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%116%Б%базовый вектор starT- представления
   {базовый вектор \sT представления}%
   {basis vector of starT representation}%
\Index%117%Б%базовый вектор Tstar- представления
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений \mathfrak{F}- алгебр
   {башня представлений $\Vector{\mathfrak{F}}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%121%Б%бесконечно малый генератор
   {бесконечно малый генератор}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\SetIndexSpace%
\Index%123%В%вектор Килинга второго рода
   {вектор Килинга второго рода}%
   {Killing vector second type}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%130%В%вырожденное аддитивное отображение D- векторного пространства
   {вырожденное аддитивное отображение $D$\Hyph векторного пространства}%
   {singular additive map, D vector space}%
\Index%131%В%вырожденное аддитивное отображение тела
   {вырожденное аддитивное отображение тела}%
   {singular additive map, division ring}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в drc векторном пространстве
   {геометрический объект в координатном представлении, определённом в \drc векторном пространстве}%
   {geometrical object, coordinate drc vector space}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometrical object of type A, vector space}%
\Index%136%Г%геометрический объект, определённый в drc векторном пространстве
   {геометрический объект, определённый в \drc векторном пространстве}%
   {geometrical object, drc vector space}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%139%Г%гомоморфизм расслоенных \mathfrak{F}- алгебр
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%149%Д%декартова степень \mathcal{A} расслоения \mathcal{B}
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power A of bundle B}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения \mathcal{E}
   {декартова степень $n$ расслоения $\mathcal{E}$}%
   {Cartesian power n of bundle E}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%156%Д%дифференциал Гато второго порядка отображения \Vector f
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Index%155%Д%дифференциал Гато второго порядка отображения f
   {дифференциал Гато второго порядка отображения $f$}%
   {Gateaux differential of Second Order, division ring}%
\Index%157%Д%дифференциал Гато отображения \Vector f нормированного D- векторного пространства \Vector{V} в нормированное D- векторное пространство \Vector{W}
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Index%158%Д%дифференциал Гато отображения f
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Index%159%Д%дуальное пространство к drc векторному пространству
   {дуальное пространство к \drc векторному пространству}%
   {dual space of drc vector space}%
\SetIndexSpace%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%161%З%закон ассоциативности для drc линейных отображений векторных пространств
   {закон ассоциативности для \drc линейных отображений векторных пространств}%
   {associative law for drc linear maps of vector spaces}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\SetIndexSpace%
\Index%266%И%изоморфизм представлений $\mathfrak{F}$\Hyph алгебры
   {изоморфизм представлений $\mathfrak{F}$\Hyph алгебры}%
   {isomorphism of repesentations of F algebra}%
\Index%173%И%изоморфизм расслоенных \mathfrak{F}- алгебр
   {изоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {isomorphism of fibered F-algebras}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений \mathfrak{F}- алгебры A
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры $A$}%
   {category of Tstar representations of F algebra}%
\Index%177%К%категория Tstar- представлений \mathfrak{F}- алгебры из категории A
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of F algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%192%К%компонента линейного отображения D- векторного пространчства
   {компонента линейного отображения $D$\Hyph векторного пространчства}%
   {component of linear map, D vector space}%
\Index%193%К%компонента линейного отображения f тела
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Index%194%К%компонента полиаддитивного отображения \Vector A
   {компонента полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Index%195%К%компонента полилинейного отображения тела
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Index%196%К%компонента производной Гато второго порядка отображения \Vector f(\Vector x)
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Index%197%К%компонента производной Гато второго порядка отображения тела
   {компонента производной Гато второго порядка отображения тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Index%199%К%компонента производной Гато отображения \Vector f(\Vector x)
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Index%198%К%компонента производной Гато отображения f(x)
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%204%К%координатная матрица вектора в drc базисе
   {координатная матрица вектора в \drc базисе}%
   {coordinate matrix of vector in drc basis}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов в векторном пространстве dcr строк
   {координатная матрица множества векторов в векторном пространстве \dcr строк}%
   {coordinate matrix of set of vectors, dcr vector space}%
\Index%207%К%координатная матрица множества векторов в векторном пространстве drc строк
   {координатная матрица множества векторов в векторном пространстве \drc строк}%
   {coordinate matrix of set of vectors, drc vector space}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%209%К%координатное drc векторное пространство
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%212%К%координатное представление в drc векторном пространстве
   {координатное представление в \drc векторном пространстве}%
   {coordinate representation, drc vector space}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный drc изоморфизм
   {координатный \drc изоморфизм}%
   {coordinate drc isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%323%К%координаты автоморфизма представления
   {координаты автоморфизма представления}%
   {coordinates of automorphism of representation}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора в drc базисе
   {координаты вектора в \drc базисе}%
   {coordinates of vector in drc basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometrical object, vector space}%
\Index%219%К%координаты геометрического объекта в drc векторном пространстве
   {координаты геометрического объекта в \drc векторном пространстве}%
   {coordinates of geometrical object, drc vector space}%
\Index%220%К%координаты геометрического объекта в координатном drc векторном пространстве
   {координаты геометрического объекта в координатном \drc векторном пространстве}%
   {coordinates of geometrical object, coordinate drc vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometrical object, coordinate vector space}%
\Index%222%К%координаты множества векторов в dcr векторном пространстве
   {координаты множества векторов в \dcr векторном пространстве}%
   {coordinates of set of vectors, dcr vector space}%
\Index%223%К%координаты множества векторов в drc векторном пространстве
   {координаты множества векторов в \drc векторном пространстве}%
   {coordinates of set of vectors, drc vector space}%
\Index%571%К%координаты пассивного отображения многообразия базисов представления
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%558%К%координаты элемента относительно множества
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление \mathfrak{F}- алгебры A в H алгебре M
   {левостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в $\mathfrak{H}$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной \mathfrak{F}- алгебры
   {левостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {left-side representation of fibered F-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%237%Л%левый модуль
   {левый модуль}%
   {left module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%241%Л%линейное отображение D- векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map, vector space}%
\Index%242%Л%линейное отображение D- векторных пространств над полем F
   {линейное отображение $D$\Hyph векторных пространств над полем $F$}%
   {linear map over field, vector space}%
\Index%243%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map, division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\Index%568%Л%лупа автоморфизмов представления
   {лупа автоморфизмов представления}%
   {loop of automorphisms of representation}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%584%М%матрица Astar линейного отображения
   {матрица $A\star$\Hyphc линейного отображения}%
   {matrix of Astar linear map}%
\Index%251%М%матрица drc линейного отображения
   {матрица \drc линейного отображения}%
   {matrix of drc linear map}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов H алгебры
   {матрица эндоморфизмов $\mathfrak{H}$\Hyph алгебры}%
   {matrix of endomorphisms of H algebra}%
\Index%527%М%матрица Якоби Гато отображения D- векторного пространства
   {матрица Якоби\Hyph Гато отображения $D$\Hyph векторного пространства}%
   {Jacobi Gateaux matrix of map, D vector space}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие drc базисов аффинного пространства
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Index%255%М%многообразие базисов drc векторного пространства
   {многообразие базисов \drc векторного пространства}%
   {basis manifold of drc vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%264%М%морфизм Tstar- представлений расслоенной \mathfrak{F}- алгебры
   {морфизм \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {morphism of representations of fibered F algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений \mathfrak{F}- алгебры в \mathfrak{H}- алгебре
   {морфизм представлений $\mathfrak{F}$\Hyph алгебры в $\mathfrak{H}$\Hyph алгебре}%
   {morphism of representations of F algebra in H algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%269%М%морфизм расслоенных Tstar- представлений из \mathcal{F} в \mathcal{G}
   {морфизм расслоенных \Ts представлений из $\mathcal{F}$ в $\mathcal{G}$}%
   {morphism of fibered representations from f into g}%
\SetIndexSpace%
\Index%270%Н%направление в D- векторном пространстве \Vector V над полем P
   {направление в $D$\Hyph векторном пространстве $\Vector V$ над полем $P$}%
   {direction over field, D vector space}%
\Index%271%Н%направление в теле D над коммутативным кольцом P
   {направление в теле $D$ над коммутативным кольцом $P$}%
   {direction over commutative ring, ring}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывная функция тела
   {непрерывная функция тела}%
   {continuous function, division ring}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%285%Н%норма отображения  тела
   {норма отображения  тела}%
   {norm of map, division ring}%
\Index%286%Н%норма отображения \Vector A нормированного D-векторного пространства
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Index%287%Н%нормированное D- векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\SetIndexSpace%
\Index%289%О%образующая аддитивного отображения
   {образующая аддитивного отображения}%
   {generator of additive map, division ring}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%297%О%однотранзитивное представление \mathfrak{F}- алгебры A
   {однотранзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной \mathfrak{F}- алгебры
   {однотранзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {single transitive representation of fibered F-algebra}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%307%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормальный базис
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%310%О%отображение D- векторного пространства, мультипликативное над полем
   {отображение $D$\Hyph векторного пространства, мультипликативное над полем}%
   {map multiplicative over field, D vector space}%
\Index%311%О%отображение D- векторного пространства, проективное над полем
   {отображение $D$\Hyph векторного пространства, проективное над полем}%
   {map projective over field, D vector space}%
\Index%312%О%отображение колец R_1, ..., R_n, полилинейное над коммутативным кольцом P
   {отображение полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%313%О%отображение кольца D, линейное над коммутативным кольцом F
   {отображение кольца $D$, линейное над коммутативным кольцом $F$}%
   {linear map over commutative ring, ring}%
\Index%314%О%отображение кольца, мультипликативное над коммутативным кольцом
   {отображение кольца, мультипликативное над коммутативным кольцом}%
   {map multiplicative over commutative ring, ring}%
\Index%315%О%отображение кольца, проективное над коммутативным кольцом
   {отображение кольца, проективное над коммутативным кольцом}%
   {map projective over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное Tstar- представление
   {пассивное \Ts представление}%
   {passive Tstar representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве drc базисов
   {пассивное преобразование на множестве \drc базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%342%П%полиаддитивное отображение (n)-D-векторных пространств
   {полиаддитивное отображение $(n)$\hyph $D$\hyph векторных пространств}%
   {polyadditive map of D vector spaces}%
\Index%343%П%полиаддитивное отображение колец
   {полиаддитивное отображение колец}%
   {polyadditive map of rings}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric, division ring}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%346%П%полилинейное отображение колец
   {полилинейное отображение колец}%
   {polylinear map of rings}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric, division ring}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%351%П%последовательность Коши в нормированное теле
   {последовательность Коши в нормированное теле}%
   {Cauchy sequence, valued division ring}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление \mathfrak{F}- алгебры A в H алгебре M
   {правостороннее представление $\mathfrak{F}$\Hyph алгебры $A$ в $\mathfrak{H}$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной \mathfrak{F}- алгебры
   {правостороннее представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {right-side representation of fibered F-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%361%П%правый модуль
   {правый модуль}%
   {right module}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%364%П%предел последовательности в нормированном теле
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%368%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometrical object, drc vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometrical object, vector space}%
\Index%371%П%представление \mathfrak{F}- алгебры A в H алгебре M
   {представление $\mathfrak{F}$\Hyph алгебры $A$ в $\mathfrak{H}$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%370%П%представление \mathfrak{F}- алгебры A в категории B
   {представление $\mathfrak{F}$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of F algebra in category}%
\Index%529%П%представление F- алгебры в башне представлений
   {представление $\mathcal F$\Hyph алгебры в башне представлений}%
   {representation of F algebra in tower of representations}%
\Index%528%П%представление F$ алгебры в представлении
   {представление $\mathcal F$\Hyph алгебры в представлении}%
   {representation of F algebra in representation}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%374%П%преобразование H алгебры
   {преобразование $\mathfrak{H}$\Hyph алгебры}%
   {transformation of H algebra}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в \mathcal{A}
   {приведенное расслоенное соответствие в $\mathcal{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из \mathcal{A} в \mathcal{B}
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%384%П%принцип инвариантности
   {принцип инвариантности}%
   {invariance principle}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%387%П%проекция расслоения \mathcal{E} вдоль слоя E
   {проекция расслоения $\mathcal{E}$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometrical object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometrical object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной \mathfrak{F}- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of fibered F algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений \mathfrak{F}- алгебры
   {произведение морфизмов представлений $\mathfrak{F}$\Hyph алгебры}%
   {product of morphisms of representations of F algebra}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка отображения f
   {производная Гато второго порядка отображения $f$}%
   {Gateaux derivative of Second Order, division ring}%
\Index%398%П%производная Гато отображения \Vector f нормированого D- векторного пространства \Vector{V} в нормированное D- векторное пространство \Vector{W}
   {производная Гато отображения $\Vector f$ нормированого $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Index%397%П%производная Гато отображения f
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Index%399%П%производная Гато порядка n отображения \Vector f
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Index%400%П%производная Гато порядка n отображения f тела
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение drc векторных пространств
   {прямое произведение \drc векторных пространств}%
   {direct product, drc vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%417%Р%размерность drc векторного пространства
   {размерность \drc векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная \mathfrak{F}- алгебра
   {расслоенная $\mathfrak{F}$\Hyph алгебра}%
   {fibered F-algebra}%
\Index%421%Р%расслоенная \mathfrak{F}- подалгебра
   {расслоенная $\mathfrak{F}$\Hyph подалгебра}%
   {fibered F-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в \mathcal{A}
   {расслоенное соответствие в $\mathcal{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из \mathcal{A} в \mathcal{B}
   {расслоенное соответствие из $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения \mathcal{A} в \mathcal{B}
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of linear equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%453%С%смешанная частная производная Гато отображения f^j по переменным v^i, v^j
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%456%С%стандартная F- компонента аддитивного отображения f
   {стандартная $F$\Hyph компонента аддитивного отображения $f$}%
   {standard component of additive map, division ring}%
\Index%458%С%стандартная компонента дифференциала Гато отображения f
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Index%459%С%стандартная компонента квадратичного отображения f над полем F
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Index%460%С%стандартная компонента линейного отображения тела
   {стандартная компонента линейного отображения тела}%
   {standard component of linear map, division ring}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения f тела
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%
\Index%574%С%стандартная компонента тензора в тензорном произведении алгебр
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Index%464%С%стандартное F- представление аддитивного отображения тела
   {стандартное $F$\Hyph представление аддитивного отображения тела}%
   {additive map, standard representation, division ring}%
\Index%465%С%стандартное представление дифференциала Гато отображения тела над полем F
   {стандартное представление дифференциала Гато отображения тела над полем $F$}%
   {Gateaux differential, standard representation, division ring}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%467%С%стандартное представление линейного отображения тела
   {стандартное представление линейного отображения тела}%
   {linear map, standard representation, division ring}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения тела
   {стандартное представление полилинейного отображения тела}%
   {polylinear map, standard representation, division ring}%
\Index%471%С%стандартные координаты drc базиса
   {стандартные координаты \drc базиса}%
   {standard coordinates of drc basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%473%С%структурные константы тела D над полем F
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%475%С%сумма drc линейных отображений
   {сумма \drc линейных отображений}%
   {sum of drc linear maps, drc vector spaces}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometrical objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometrical objects, vector space}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%487%Т%топологическое drc векторное пространство
   {топологическое \drc векторное пространство}%
   {topological drc vector space}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление \mathfrak{F}- алгебры A
   {транзитивное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной \mathfrak{F}- алгебры
   {транзитивное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {transitive representation of fibered F-algebra}%
\SetIndexSpace%
\Index%493%У%уравнение Килинга
   {уравнение Килинга}%
   {Killing equation}%
\Index%494%У%уравнение Килинга второго рода
   {уравнение Килинга второго рода}%
   {Killing equation second type}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр \mathfrak{F} сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%500%Ф%фундаментальная последовательность в нормированное теле
   {фундаментальная последовательность в нормированное теле}%
   {fundamental sequence, valued division ring}%
\Index%588%Ф%функциональная матрица
   {функциональная матрица}%
   {functional matrix}%
\Index%502%Ф%функция \gi n D- значных переменных
   {функция $\gi n$ $D$\Hyph значных переменных}%
   {function of n D valued variables}%
\Index%501%Ф%функция D- векторного пространства \Vector{V} в D- векторное пространство \Vector W, дифференцируемая по Гато
   {функция $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector W$, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, D vector space}%
\Index%503%Ф%функция проективна над полем R и непрерывна по направлению над полем R
   {функция проективна над полем $R$ и непрерывна по направлению над полем $R$}%
   {projective function is continuous in direction over field R, division ring}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%505%Ф%функция тела, дифференцируемая по Гато
   {функция тела, дифференцируемая по Гато}%
   {function differentiable in Gateaux sense, division ring}%
\Index%506%Ф%функция, непрерывная по совокупности аргументов
   {функция, непрерывная по совокупности аргументов}%
   {function continuous with respect to set of arguments}%
\SetIndexSpace%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%510%Ч%частная crd производная Гато отображения {}^bf по переменной {}^ax
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map with respect to variable, D vector space}%
\Index%511%Ч%частная drc производная Гато отображения f^b по переменной x^a
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато отображения f^j по переменной v^i
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Index%513%Ч%частное аддитивное отображение переменной v^i
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления F алгебры
   {эндоморфизм представления $\mathfrak{F}$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%324%Э%эффективная башня Tstar- представлений
   {эффективная башня \Ts представлений}%
   {effective tower of representations}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление \mathfrak{F}- алгебры A
   {эффективное представление $\mathfrak{F}$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%519%Э%эффективное представление расслоенной \mathfrak{F}- алгебры
   {эффективное представление расслоенной $\mathfrak{F}$\Hyph алгебры}%
   {effective representation of fibered F-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%522%Я%ядро аддитивного отображения D- векторного пространства
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Index%523%Я%ядро аддитивного отображения тела
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%

\CloseIndex


==> Preface.1001.4852.Russian.tex <==
%auto-ignore
\input{Preface.1001.4852.Eq}

\section{Предисловие}

Я дал определение тензорного произведения тел
(раздел
\xRef{0701.238}{section: Tensor Product of Division Rings})
практически одновременно с определением линейного отображения
тел (раздел
\xRef{0701.238}{section: Additive Map of Division Ring}).
Для меня было очевидно, что компоненты линейного отображения
были тензором валентности $2$. Но этот факт был для
меня настолько неожиданным, что я до сих пор ничего не
писал об этом в своих статьях.

В этом утверждение было некоторое противоречие.
Я использовал линейное отображение, чтобы определить тензор
валентности $1$, а для построения отображения мне нужен был
тензор валентности $2$, т. е. билинейное отображение.

Никакого парадокса, однако, здесь нет.
Для любого поля $F$ тензорное произведение $F\otimes F$
изоморфно $F$. Следствием этого изоморфизма является возможность
заменить тензор $a\otimes b$ обычным произведением $ab$.
Поэтому множество линейных отображений поля $F$ изоморфно
полю $F$, или точнее, множеству левых сдвигов мультипликативной
группы поля $F$.
В теле произведение некоммутативно и этот изоморфизм отсутствует.

Другая проблема, с которой я встретился, возникла, когда я
захотел представить производную отображения векторных пространств
в виде матрицы частных производных (равенство
\xEqRef{0812.4763}{eq: Jacobi Gateaux matrix of map, D vector space}).
Возникает желание записать матрицу Якоби\Hyph Гато отображения
в виде произведения матриц
\ShowEq{Jacobi Gateaux matrix of map, vector space}
Однако очевидно, что равенство
\eqref{eq: Jacobi Gateaux matrix of map, vector space}
неверно.
Однако матрица, записанная в левой части равенства
\eqref{eq: Jacobi Gateaux matrix of map, vector space}
имеет очень серьёзный недостаток.
Возникает ощущение, что ранг этой матрицы зависит от приращения аргумента.

Похожая картина наблюдается в теореме
\xRef{0812.4763}{theorem: composite map, differential, D vector space},
где производная имеет вид
\ShowEq{differential of composite map, D vector space}

Последним доводом изменить рассматриваемую модель
стал закон преобразования вектора
в криволинейых координатах аффинного пространства
(равенства
\xEqRef{0906.0135}{eq: map and coordinates, 5, D affine space},
\xEqRef{0906.0135}{eq: map and coordinates, 6, D affine space})
\ShowEq{map and coordinates, D affine space}
Это меня окончательно убедило в том, что я встретил новый математический
объект. Имя этого объекта функциональная матрица, т. е. матрица,
элементами которой являются отображения.

%Произведение функциональных матриц отличается от произведения
%обычных матриц тем, что вместо произведения элемента одной матрицы
%на элемент другой я рассматриваю произведение соответствующих
%отображений.
%Чтобы подчеркнуть это отличие, я предложил
%новую запись для произведения функциональных матриц.

Осталось сделать последний шаг. Если элемент матрицы отображение,
то я разрываю связь между отображением и аргументом, точнее говоря,
я записываю отображение как оператор
\ShowEq{new notation for mapping}

В новых обозначениях линейное отображение тела можно записать в виде
\ShowEq{linear mapping of division ring}
Соответственно, производную отображения $f$ можно записать в виде
\ShowEq{derivative of mapping f}
В равенстве \eqref{eq: derivative of mapping f}
мне удалось разделить производную и приращение.


==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%A%0
\Symb%
   {$(^a_b)$\hyph\CR квазидетерминант}%
   {a b CR quasideterminant definition}%
\Symb%
   {$(^a_b)$\hyph \RC квазидетерминант}%
   {a b RC-quasideterminant definition}%
\Symb%
   {$(^a_b)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {a b RCcirc-quasideterminant definition}%
\Symb%
   {минор}%
   {A from b a}%
\Symb%
   {минор}%
   {A from columns T}%
\Symb%
   {минор}%
   {A from rows S}%
\Symb%
   {минор}%
   {A without column a}%
\Symb%
   {минор}%
   {A without columns T}%
\Symb%
   {минор}%
   {A without row b}%
\Symb%
   {минор}%
   {A without rows S}%
\Symb%
   {аффинное пространство}%
   {affine space, division ring}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {компонента линейного отображения $\Vector{A}$ $D$\Hyph векторного пространства}%
   {component of linear map, D vector space}%
\Symb%
   {компонента $p$ полиаддитивного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {\dcr вектор}%
   {dcr vector}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {лупа автоморфизмов представления $f$}%
   {loop of automorphisms of representation}%
\Symb%
   {норма отображения $\Vector A$ нормированного $D$\hyph векторного пространства}%
   {norm of map, D vector space}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное аддитивное отображение переменной $v^i$}%
   {partial additive map of variable}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {множество аддитивных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set additive maps, D vector space}%
\Symb%
   {множество аддитивных отображений кольца $R_1$ в кольцо $R_2$}%
   {set additive maps, ring}%
\Symb%
   {множество полиаддитивных отображений}%
   {set polyadditive maps, D vector space}%
\Symb%
   {множество полиаддитивных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polyadditive maps, ring}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {стандартная компонента тензора в тензорном произведении алгебр}%
   {standard component of tensor, algebra}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \drc векторного пространства $\mathcal{V}$}%
   {basis manifold of drc vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {декартова степень $\mathcal{A}$ расслоения $\mathcal{B}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {многообразие \drc базисов аффинного пространства}%
   {drc Basis Manifold, Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {структурные константы тела $D$ над полем $F$}%
   {structural constants of division ring over field}%

\SetIndexSpace%C%0
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {$\CRcirc$\Hyph произведение функциональных матриц}%
   {cr product of functional matrices}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation}%
\Symb%
   {базовый вектор \Ts представления}%
   {basis vector of starT representation, coordinates}%
\Symb%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation}%
\Symb%
   {базовый вектор \Ts представления}%
   {basis vector of Tstar representation, coordinates}%
\Symb%
   {\dcr векторное пространство \subs строк}%
   {c rows dcr vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space}%
\Symb%
   {компонента производной Гато отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, division ring}%
\Symb%
   {компонента производной Гато второго порядка отображения $\Vector f(\Vector x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$ тела}%
   {component of Gateaux derivative of Second Order, division ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \drc векторное пространство}%
   {coordinate drc vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\crd производная Гато отображения $\Vector f$ $D$\hyph векторного пространства $\Vector V$ в $D$\hyph векторное пространство $\Vector W$}%
   {Gateaux crd derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, division ring}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $\Vector f$}%
   {Gateaux derivative of Order n, D vector space}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка отображения $\Vector f$}%
   {Gateaux derivative of Second Order, D vector space}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, division ring}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $\Vector f$ нормированного $D$\Hyph векторного пространства $\Vector{V}$ в нормированное $D$\Hyph векторное пространство $\Vector{W}$}%
   {Gateaux differential of map, D vector space}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, division ring}%
\Symb%
   {дифференциал Гато второго порядка отображения $\Vector f$}%
   {Gateaux differential of Second Order, D vector space}%
\Symb%
   {дифференциал Гато второго порядка отображения $f$ тела}%
   {Gateaux differential of Second Order, division ring}%
\Symb%
   {\drc производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $\Vector V$ в $D$\Hyph векторное пространство $\Vector W$}%
   {Gateaux drc derivative of map, D vector space}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 1, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 2, D vector space}%
\Symb%
   {частная \crd производная Гато отображения ${}^bf$ по переменной ${}^ax$}%
   {Gateaux partial crd derivative of map, 3, D vector space}%
\Symb%
   {смешанная частная производная Гато отображения $f^j$ по переменным $v^i$, $v^j$}%
   {Gateaux partial derivative of Second Order, D vector space}%
\Symb%
   {частная производная Гато отображения $f^j$ по переменной $v^i$}%
   {Gateaux partial derivative, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 1, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 2, D vector space}%
\Symb%
   {частная \drc производная Гато отображения $f^b$ по переменной $x^a$}%
   {Gateaux partial drc derivative of map, 3, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {\drc векторное пространство \sups строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента дифференциала Гато отображения $f$}%
   {standard component of Gateaux differential, division ring}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\mathcal{V}$}%
   {basis in V}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {аффинный базис}%
   {drc affine basis, division ring}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\mathcal{E}$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\mathcal{E}$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {активное представление лупы $\mathfrak A(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {координаты базиса в \dcr векторном пространстве \subs строк}%
   {basis coordinates, c rows dcr vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \sups строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \dcr векторном пространстве \subs строк}%
   {basis, c rows dcr vector space}%
\Symb%
   {базис в \drc векторного пространства \sups строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения тела}%
   {component of polylinear map, division ring}%
\Symb%
   {расслоенный морфизм из расслоения $\mathcal{A}$ в $\mathcal{B}$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных $\mathfrak{F}$\Hyph алгебр}%
   {homomorphism of fibered F-algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма отображения $f$  тела}%
   {norm of map, division ring}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормальный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная $F$\Hyph компонента аддитивного отображения $f$ }%
   {standard component of additive map, division ring}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения $f$ тела}%
   {standard component of linear map, division ring}%
\Symb%
   {стандартная компонента полилинейного отображения $f$ тела}%
   {standard component of polylinear map, division ring}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor, division ring}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {группа аффинных преобразований}%
   {drc affine transformation group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа гомоморфизмов векторного пространства $\mathcal{V}$}%
   {GV}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро аддитивного отображения $D$\Hyph векторного пространства}%
   {kernel of additive map, D vector space}%
\Symb%
   {ядро аддитивного отображения тела}%
   {kernel of additive map, division ring}%

\SetIndexSpace%L%0
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности в нормированном теле}%
   {limit of sequence, valued division ring}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {\rcd векторное пространство \drc линейных отображений \drc векторного пространства $\Vector{V}$ в \drc векторное пространство $\Vector{W}$}%
   {set drc linear maps, drc vector space}%
\Symb%
   {множество линейных отображений $D$\Hyph векторного пространства $\Vector{V}$ в $D$\Hyph векторное пространство $\Vector{W}$}%
   {set linear maps, D vector space}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {\drc векторное пространство \rcd линейных отображений \rcd векторного пространства $\Vector{V}$ в \rcd векторное пространство $\Vector{W}$}%
   {set rcd linear maps, rcd vector space}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований множества $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \drc векторном пространстве}%
   {geometrical object, coordinate drc vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometrical object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \drc векторном пространстве}%
   {geometrical object, drc vector space}%
\Symb%
   {орбита представления расслоенной группы $\mathcal{G}$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень расслоения}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\mathcal{A}$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {\Ds компонента координат вектора $\Vector r$}%
   {Dstar component of coordinates of vector, D vector space}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение функциональных матриц}%
   {rc product of functional matrices}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%
\Symb%
   {\sD компонента координат вектора $\Vector r$}%
   {starD component of coordinates of vector, D vector space}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры $A$}%
   {category of Tstar representations of F algebra}%
\Symb%
   {категория \Ts представлений $\mathfrak{F}$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of F algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%

\SetIndexSpace%V%0
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, drc vector space, 1 n}%
\Symb%
   {дуальное пространство к \drc векторному пространству $\Vector V$}%
   {dual space of drc vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {\dcr векторное пространство}%
   {left CR vector space}%
\Symb%
   {\drc векторное пространство}%
   {left RC vector space}%
\Symb%
   {\crd векторное пространство}%
   {right CR vector space}%
\Symb%
   {\rcd векторное пространство}%
   {right RC vector space}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J_f(X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {координаты пассивного отображения многообразия базисов представления}%
   {coordinates of passive map of basis manifold of representation}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometrical object, vector space}%

\SetIndexSpace%X%0
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {базовый оператор группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, drc vector space}%
\Symb%
   {прямое произведение $D_i\RCstar$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, drc vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

